Customs Fraud Detection in the Presence of Concept Drift

Capturing the changing trade pattern is critical in customs fraud detection. As new goods are imported and novel frauds arise, a drift-aware fraud detection system is needed to detect both known frauds and unknown frauds within a limited budget. The current paper proposes ADAPT, an adaptive selection method that controls the balance between exploitation and exploration strategies used for customs fraud detection. ADAPT makes use of the model performance trends and the amount of concept drift to determine the best exploration ratio at every time. Experiments on data from four countries over several years show that each country requires a different amount of exploration for maintaining its fraud detection system. We find the system with ADAPT can gradually adapt to the dataset and find the appropriate amount of exploration ratio with high performance.

==> tables/deprecated/results_target_c.tex <==
\begin{table}[h!]
\centering
% \scriptsize
\caption{Customs selection performance in Country C boosted significantly by using additional countries datasets and domain adaptation technique.}
\label{tab:datastats}
% \resizebox{\linewidth}{!}{%
\begin{tabular}{p{2cm} p{1.3cm} p{1.3cm} p{1.3cm} p{1.3cm}} \toprule
    Source and target ($c_s \rightarrow c_t$) & DATE \newline ($c_t$ only) & DATE \newline ($c_s + c_t$) & Other SOTA \newline ($c_s + c_t$) & Domain \newline Adaptation \newline ($c_s + c_t$)  \\ \midrule
    \textsf{M} $\rightarrow$ \textsf{C} & & & & \\
    \textsf{N} $\rightarrow$ \textsf{C} & & & & \\
    \textsf{T} $\rightarrow$ \textsf{C} & & & & \\
    \textsf{M}$+$\textsf{N} $\rightarrow$ \textsf{C} & & & & \\
    \textsf{M}$+$\textsf{T} $\rightarrow$ \textsf{C} & & & & \\
    \textsf{N}$+$\textsf{T} $\rightarrow$ \textsf{C} & & & & \\
    \textsf{M}$+$\textsf{N}$+$\textsf{T} $\rightarrow$ \textsf{C} & & & & \\
    \bottomrule
\end{tabular}
% }
\end{table}

==> tables/deprecated/results_target_m.tex <==
\begin{table}[h!]
\centering
% \scriptsize
\caption{Customs selection performance in Country M boosted significantly by using additional countries datasets and domain adaptation technique.}
\label{tab:datastats}
% \resizebox{\linewidth}{!}{%
\begin{tabular}{p{2cm} p{1.3cm} p{1.3cm} p{1.3cm} p{1.3cm}} \toprule
    Source and target ($c_s \rightarrow c_t$) & DATE \newline ($c_t$ only) & DATE \newline ($c_s + c_t$) & Other SOTA \newline ($c_s + c_t$) & Domain \newline Adaptation \newline ($c_s + c_t$)  \\ \midrule
    \textsf{N} $\rightarrow$ \textsf{M} & 0.0581 & 0.5055 & & 0.6320 \\
    \textsf{C} $\rightarrow$ \textsf{M} & & & & \\
    \textsf{T} $\rightarrow$ \textsf{M} & & & & \\
    \textsf{N}$+$\textsf{T} $\rightarrow$ \textsf{M} & & & & \\
    \textsf{N}$+$\textsf{C} $\rightarrow$ \textsf{M} & & & & \\
    \textsf{C}$+$\textsf{T} $\rightarrow$ \textsf{M} & & & & \\
    \textsf{N}$+$\textsf{C}$+$\textsf{T} $\rightarrow$ \textsf{M} & & & & \\ \bottomrule
\end{tabular}
% }
\end{table}

==> tables/deprecated/results_target_n.tex <==
\begin{table}[h!]
\centering
% \scriptsize
\caption{Customs selection performance in Country M boosted significantly by using additional countries datasets and domain adaptation technique.}
\label{tab:datastats}
% \resizebox{\linewidth}{!}{%
\begin{tabular}{p{2cm} p{1.3cm} p{1.3cm} p{1.3cm} p{1.3cm}} \toprule
    Source and target ($c_s \rightarrow c_t$) & DATE \newline ($c_t$ only) & DATE \newline ($c_s + c_t$) & Other SOTA \newline ($c_s + c_t$) & Domain \newline Adaptation \newline ($c_s + c_t$)  \\ \midrule
    \textsf{M} $\rightarrow$ \textsf{N} & & & & \\
    \textsf{C} $\rightarrow$ \textsf{N} & & & & \\
    \textsf{T} $\rightarrow$ \textsf{N} & & & & \\
    \textsf{M}$+$\textsf{C} $\rightarrow$ \textsf{N} & & & & \\
    \textsf{M}$+$\textsf{C} $\rightarrow$ \textsf{N} & & & & \\
    \textsf{M}$+$\textsf{C} $\rightarrow$ \textsf{N} & & & & \\
    \textsf{M}$+$\textsf{C}$+$\textsf{T} $\rightarrow$ \textsf{N} & & & & \\
    \bottomrule
\end{tabular}
% }
\end{table}

==> tables/methods.tex <==

\begin{table}[h!]
\small
\resizebox{\columnwidth}{!}{  

\begin{tabular}[t]{p{0.15\columnwidth}p{0.82\columnwidth}}
\toprule
Method & Description \\ \midrule

Naive approach & This approach use the uncertainty coefficient defined by the change in importer IDs, averaged with FOB price change over time. Although this approach is simple, it cannot consider complex data patterns. 
% \newline \textit{Output:} Value in [0; 1] indicating the amount of concept shift. 
\\ \midrule

Statistical \newline approach & This approach uses statistical tests to measure difference in distributions over time and correlated p-value to measure the concept shift amount. Kolomogorov-Smirnov, t-test, and Anderson-Darling tests can be used. However, this approach only considers numerical features, and it is sensitive to the number of available samples~\cite{KSandAD}.
% \newline \textit{Output:} Value in [0; 1] indicating the amount of concept shift. 
\\ \midrule

Optimal \newline transport & Optimal transport transforms one data distribution into another and utilizes the cost needed for transformation as a concept drift amount~\cite{OTML}. The data imbalance requires under/oversampling, causing loss of information. More complex transformation functions are needed to have a closer transformation result.
% \newline \textit{Output:} Value in [$-\infty$; $\infty$] indicating the amount of concept shift.
 \\ \midrule

Clustering-based approach & How to distinguish new data points into normal, concept drift, or novelty? We can cluster normal data points and compare a new transaction to the existing clusters to decide if it is normal, shift, or novelty~\cite{olindda}. Although we can directly cluster the raw data, clustering might be sensitive to the sparseness and the number of data samples. 
% Utilize this division when retraining the model to account for concept shift excluding anomalies. % \newline \textit{Output:} New data points are labeled as normal, concept shift, or novelty. \newline \textit{Limitation:} 
\\ \bottomrule
\end{tabular}
}
\caption{Four methodologies to measure concept drift in import trades.}
\label{tab:summary}
\end{table}

==> tables/results_main.tex <==
\begin{table}[t]
\centering
% \scriptsize
\caption{Example table from Ryan's experiments}
\label{tab:results_main}
% \resizebox{\linewidth}{!}{%
\begin{tabular}{p{2cm} p{1.3cm} p{1.3cm} p{1.3cm} p{1.3cm}} \toprule
    Source and target ($c_s \rightarrow c_t$) & DATE \newline ($c_t$ only) & DATE \newline ($c_s + c_t$) & Other SOTA \newline ($c_s + c_t$) & Domain \newline Adaptation \newline ($c_s + c_t$)  \\ \midrule
    \textsf{N} $\rightarrow$ \textsf{M} & 0.0796 & 0.6391 & & 0.6738 \\
    \textsf{C} $\rightarrow$ \textsf{M} & & 0.4455& &  0.5123\\
    \textsf{T} $\rightarrow$ \textsf{M} &  & 0.3323 & & 0.5124 \\
    \textsf{N}$+$\textsf{T} $\rightarrow$ \textsf{M} & & & & \\
    \textsf{N}$+$\textsf{C} $\rightarrow$ \textsf{M} & & & & \\
    \textsf{C}$+$\textsf{T} $\rightarrow$ \textsf{M} & & & & \\
    \textsf{N}$+$\textsf{C}$+$\textsf{T} $\rightarrow$ \textsf{M} & & & &
    \\
    \midrule
    \textsf{M} $\rightarrow$ \textsf{C} & 0.2213 & 0.2257 & & 0.2109 \\
    \textsf{N} $\rightarrow$ \textsf{C} & & 0.1794 & & 0.2014\\
    \textsf{T} $\rightarrow$ \textsf{C} & & 0.1707 & & 0.1720 \\
    \textsf{M}$+$\textsf{N} $\rightarrow$ \textsf{C} & & & & \\
    \textsf{M}$+$\textsf{T} $\rightarrow$ \textsf{C} & & & & \\
    \textsf{N}$+$\textsf{T} $\rightarrow$ \textsf{C} & & & & \\
    \textsf{M}$+$\textsf{N}$+$\textsf{T} $\rightarrow$ \textsf{C} & & & & \\ \midrule
    \textsf{M} $\rightarrow$ \textsf{N} & 0.7513 & 0.7452 & & 0.7567\\
    \textsf{C} $\rightarrow$ \textsf{N} & & 0.6812 & & 0.7121 \\
    \textsf{T} $\rightarrow$ \textsf{N} & & 0.5475 & &  0.6956\\
    \textsf{M}$+$\textsf{C} $\rightarrow$ \textsf{N} & & & & \\
    \textsf{M}$+$\textsf{C} $\rightarrow$ \textsf{N} & & & & \\
    \textsf{M}$+$\textsf{C} $\rightarrow$ \textsf{N} & & & & \\
    \textsf{M}$+$\textsf{C}$+$\textsf{T} $\rightarrow$ \textsf{N} & & & & \\ \midrule
    \textsf{M} $\rightarrow$ \textsf{T} & 0.2813 & 0.2818 & & 0.3186 \\
    \textsf{C} $\rightarrow$ \textsf{T} & & 0.2603 & & 0.3033\\
    \textsf{N} $\rightarrow$ \textsf{T} & & 0.2558 &  & 0.3047\\
    \textsf{M}$+$\textsf{C} $\rightarrow$ \textsf{T} & & & & \\
    \textsf{M}$+$\textsf{N} $\rightarrow$ \textsf{T} & & & & \\
    \textsf{C}$+$\textsf{N} $\rightarrow$ \textsf{T} & & & & \\
    \textsf{M}$+$\textsf{C}$+$\textsf{N} $\rightarrow$ \textsf{T} & & & & \\ \bottomrule
\end{tabular}
% }
\end{table}
